Non-uniformity is All You Need: Efficient and Timely Encrypted Traffic Classification With ECHO

With 95% of Internet traffic now encrypted, an effective approach to classifying this traffic is crucial for network security and management. This paper introduces ECHO -- a novel optimization process for ML/DL-based encrypted traffic classification. ECHO targets both classification time and memory utilization and incorporates two innovative techniques. The first component, HO (Hyperparameter Optimization of binnings), aims at creating efficient traffic representations. While previous research often uses representations that map packet sizes and packet arrival times to fixed-sized bins, we show that non-uniform binnings are significantly more efficient. These non-uniform binnings are derived by employing a hyperparameter optimization algorithm in the training stage. HO significantly improves accuracy given a required representation size, or, equivalently, achieves comparable accuracy using smaller representations. Then, we introduce EC (Early Classification of traffic), which enables faster classification using a cascade of classifiers adapted for different exit times, where classification is based on the level of confidence. EC reduces the average classification latency by up to 90\%. Remarkably, this method not only maintains classification accuracy but also, in certain cases, improves it. Using three publicly available datasets, we demonstrate that the combined method, Early Classification with Hyperparameter Optimization (ECHO), leads to a significant improvement in classification efficiency.

==> chapters/nonuniform/nonuniform.tex <==
\section{Hyperparameter Optimization (HO) of Binnings}
\label{sec:non-uniform}
In this section, we will present \emph{HO} (efficient classification using Hyperparameter Optimization), a novel strategy to create \emph{non-uniform binnings}. Our strategy enables efficient classification by saving memory requirements while achieving high classification accuracy.

In this work, we explored both non-uniformity in the packet size distribution vector and the arrival-time distribution vector. 
For simplicity, we describe the creation of the representation in the packet-size distribution vector, and the arrival-time distribution vector follows similarly (albeit with different parameters).

\emph{Binning} consists of reducing the granularity of the representation such that each original value is mapped to a \emph{bin}. Each bin represents an interval of the original values. 
Formally, a uniform representation of size $N$ for values in $[0,x)$  represents the data in $N$ bins, where bin $i\in\{1,\ldots,N\}$ is for values in $[\frac{(i-1)\cdot x}{N},\frac{i\cdot x}{N})$. 
A \emph{non-uniform} $N$-bin representation has additional degrees of freedom to choose the boundaries by defining a vector $$B=[b_0,\ldots,b_{N}],$$ such that  $0=b_0<b_{1}<\ldots<b_{N-1}<b_N=x$. In such a representation, bin $i\in\{1,\ldots,N\}$ is for values in $[b_{i-1} ,b_{i} )$\footnote{The last bin may map also values larger than $x$ (e.g., in case of jumbo frames), and therefore, can be defined as $[b_{N-1},\infty)$.}.

%Here, we aim to find the optimal non-uniform binning. 

Most previous research is focused on uniform representations, sometimes employing feature selection methods to reduce the granularity of data. It was also suggested to use statistical separation functions to select non-uniform bins.
% Previous research has explored non-uniformity in packet size distribution, employing methods such as feature selection and statistical separation functions.

We compare \emph{HO} with three other representation optimization methods: \emph{Uniform}, \emph{Feature Selection}, and \emph{Statistical}, which are detailed in Section \ref{sec:res:non_uniform}. Through this comparison, we demonstrate the superiority of our approach. 
Opposed to the other methods, \emph{HO} offers the highest level of flexibility in choosing variable-size bins (in contrast to \emph{Uniform} and \emph{Feature Selection}). Moreover, in \emph{HO}, the bin-selection process is tuned by the anticipated performance of the final \emph{model}, distinguishing it from \emph{Feature Selection} and \emph{Statistical}, which rely solely on data distribution. The degrees of freedom offered in each method are shown in Table \ref{tab:freedom}.
\ignore{
\begin{table}[tbp] 
% \label{tab:freedom}
    \centering
   \caption{The different parameters observable by the representation optimization process}
    \small
    \begin{tabular}{|m{1.4cm}|m{1.4cm}|m{1.5cm}|m{1.5cm}|m{0.5cm}|}
    \hline
    & \textbf{Uniform} & \textbf{Feature {Selection}} & \textbf{Statistical} & \textbf{HO} \\
    \hline
    \textbf{Data-aware} & & \centering\arraybackslash  \textcolor{green!60!black}{\ding{51}} & \centering\arraybackslash  \textcolor{green!60!black}{\ding{51}} & \centering\arraybackslash \textcolor{green!60!black}{\ding{51}} \\
    \hline
    \textbf{Variable Sized Bins} & & & \centering\arraybackslash \textcolor{green!60!black}{\ding{51}} & \centering\arraybackslash \textcolor{green!60!black}{\ding{51}} \\
    \hline
    \textbf{Model-aware} & & & & \centering\arraybackslash \textcolor{green!60!black}{\ding{51}} \\
    \hline
    \end{tabular}
    \label{tab:freedom}
\end{table}
}

\begin{table}[tbp] 
    \centering
    \caption{The different parameters observable by the representation-optimization process}
    \small
    \begin{tabular}{|m{1.5cm}|m{1.5cm}|m{1.5cm}|m{1.5cm}|}
    \hline
    \textbf{} & \textbf{Data-aware} & \textbf{Variable Sized Bins} & \textbf{Model-aware} \\
    \hline
    \textbf{Uniform} & \centering\arraybackslash \textcolor{red!60!black}{\ding{55}}& \centering\arraybackslash \textcolor{red!60!black}{\ding{55}} & \centering\arraybackslash \textcolor{red!60!black}{\ding{55}}\\
    \hline
    \textbf{Feature Selection} & \centering\arraybackslash \textcolor{green!60!black}{\ding{51}} & \centering\arraybackslash  \textcolor{red!60!black}{\ding{55}}&  \centering\arraybackslash \textcolor{red!60!black}{\ding{55}} \\
    \hline
    \textbf{Statistical} & \centering\arraybackslash \textcolor{green!60!black}{\ding{51}} & \centering\arraybackslash \textcolor{green!60!black}{\ding{51}} &  \centering\arraybackslash \textcolor{red!60!black}{\ding{55}} \\
    \hline
    \textbf{HO} & \centering\arraybackslash \textcolor{green!60!black}{\ding{51}} & \centering\arraybackslash \textcolor{green!60!black}{\ding{51}} & \centering\arraybackslash \textcolor{green!60!black}{\ding{51}} \\
    \hline
    \end{tabular}
    \label{tab:freedom}
\end{table}

In the suggested strategy, we employ 
a hyperparameter optimization algorithm.
Hyperparameter optimization refers to the process of finding the best combination of hyperparameters for a given machine-learning classifier. Hyperparameters are configuration settings that are not learned in the training stage, but rather set before training the classifier. 
We focus mainly on a Bayesian optimization approach called Tree Parzen Estimators (TPE), as it shows superiority over other approaches in past experiments~\cite{NIPS2011_86e8f7ab,pmlr-v28-bergstra13}. 
The hyperparameters for our method are the selected bins for the representation, the search space includes all possible combinations of bin boundaries, and the objective we aim to maximize in the Bayesian process is the accuracy of a trained model over the validation set.

For the experiments in this work, we used $k$-fold cross-validation (\emph{KFCV})~\cite{Kohavi1995ASO}.
Therefore, to validate the TPE process, we used nested cross-validation (NCV)~\cite{10.5555/1756006.1859921}, an extension of\emph{KFCV} for hyperparameter optimization. 
NCV consists of an outer loop for standard \emph{KFCV}, selecting training and test sets in each iteration. In the inner loop, we used the training data to iteratively select optimal hyperparameters through another \emph{KFCV} process. We used $k=5$ in both the outer and inner loops, implying that for each evaluation in the inner loop, $64\%$ of the flows are used for training, $16\%$ for validating the hyperparameters by calculating the objective function in the Bayesian process, and $20\%$ for testing (in the outer loop). It is important to note that different iterations of the outer loop might yield different hyperparameter values. 

Notice that in our settings, the optimization process is done offline on labeled data, and therefore, has fewer constraints regarding computational power or latency. 

Once the optimization process finishes and an optimal result is achieved, the real-time classifier is adapted and uses the optimal hyperparameters (namely, the bin boundaries) achieved by the offline optimizer. 

After selecting the bin boundaries, to create our representations without any computational overhead, we create a mapping, using a small direct-access array of size $x$,  between every possible packet value to its bin index; this implies that the process of building our representations (which is done online, packet by packet) does not incur additional computations (only one memory access). 

To capture changes in traffic patterns or in the underlying applications, we propose to run \emph{HO} periodically, upon degradation of accuracy, or manually if a change in the network condition is known. The process should run in the background without interfering with ongoing classifications.

The results achieved using \emph{HO}, as well as a comprehensive comparison to the alternative methods, are shown in Section \ref{sec:res:non_uniform}. 

==> chapters/results/tables/all_tasks_tables.tex <==
\small{
\begin{table}[p]
    \caption{QUIC Applications classification task.}
    \centering
    \begin{tabular}{lcccc}
    \toprule
    & {\textbf{RF}} & {\textbf{SVM}} & {\textbf{LR}} & {\textbf{DEEP}} \\
    \midrule
    \textbf{dist(5)}& \textbf{94.9\%} & 82.7\% & 93.6\% & -\\
\textbf{dist(10)}& \textbf{95.9\%} & 82.3\% & 95.5\% & -\\
\textbf{dist(20)}& \textbf{95.9\%} & 82.2\% & 95.7\% & 94.9\%\\
\underline{\textbf{dist(50)}}& 95.7\% & 79.4\% & 94.4\% & \textbf{96.2\%}\\
\textbf{ts(5)}& \textbf{94.6\%} & 81.3\% & 81.2\% & -\\
\textbf{ts(10)}& \textbf{95.1\%} & 80.5\% & 79.3\% & -\\
\textbf{ts(20)}& \textbf{95.3\%} & 84.5\% & 79.7\% & 94.7\%\\
\textbf{ts(50)}& \textbf{95.8\%} & 85.5\% & 83.8\% & 93.3\%\\
\textbf{fp(8)}& 93.0\% & 78.7\% & \textbf{95.5\%} & 95.2\%\\
\textbf{fp(16)}& 91.8\% & 69.8\% & 94.7\% & \textbf{94.7\%}\\
\textbf{fp(32)}& 90.0\% & 66.9\% & 92.5\% & \textbf{95.5\%}\\
\textbf{sts()}& \textbf{95.0\%} & 82.9\% & 90.0\% & -\\
\bottomrule
    \end{tabular}
    \label{tab:tab:Quic_Apps_table}
    \end{table}
\begin{table}[p]
    \caption{ISCX Applications classification task.}
    \centering
    \begin{tabular}{lcccc}
    \toprule
    & {\textbf{RF}} & {\textbf{SVM}} & {\textbf{LR}} & {\textbf{DEEP}} \\
    \midrule
    \textbf{dist(5)}& \textbf{80.9\%} & 73.3\% & 76.4\% & -\\
\textbf{dist(10)}& 87.0\% & 79.9\% & \textbf{91.8\%} & -\\
\textbf{dist(20)}& 87.3\% & 82.8\% & 93.4\% & \textbf{95.9\%}\\
\underline{\textbf{dist(50)}}& 88.8\% & 91.7\% & 95.6\% & \textbf{97.8\%}\\
\textbf{ts(5)}& \textbf{67.0\%} & 49.5\% & 39.1\% & -\\
\textbf{ts(10)}& \textbf{68.5\%} & 56.2\% & 42.9\% & -\\
\textbf{ts(20)}& \textbf{69.6\%} & 60.1\% & 42.8\% & 53.5\%\\
\textbf{ts(50)}& 73.7\% & 61.1\% & 42.3\% & \textbf{73.9\%}\\
\textbf{fp(8)}& \textbf{80.4\%} & 72.3\% & 77.0\% & 78.0\%\\
\textbf{fp(16)}& 81.4\% & 74.9\% & 82.6\% & \textbf{91.4\%}\\
\textbf{fp(32)}& 83.0\% & 85.3\% & 84.2\% & \textbf{94.5\%}\\
\textbf{sts()}& 92.8\% & 69.3\% & \textbf{92.9\%} & -\\
\bottomrule
    \end{tabular}
    \label{tab:tab:ISCX_Apps_table}
    \end{table}
\begin{table}[p]
    \caption{ISCX Encryption classification task.}
    \centering
    \begin{tabular}{lcccc}
    \toprule
    & {\textbf{RF}} & {\textbf{SVM}} & {\textbf{LR}} & {\textbf{DEEP}} \\
    \midrule
    \textbf{dist(5)}& \textbf{92.3\%} & 83.6\% & 81.1\% & -\\
\textbf{dist(10)}& \textbf{92.7\%} & 85.5\% & 84.1\% & -\\
\textbf{dist(20)}& 92.8\% & 88.6\% & 90.2\% & \textbf{94.6\%}\\
\underline{\textbf{dist(50)}}& 90.8\% & 93.3\% & 91.6\% & \textbf{96.2\%}\\
\textbf{ts(5)}& \textbf{81.2\%} & 68.3\% & 60.8\% & -\\
\textbf{ts(10)}& \textbf{81.9\%} & 69.8\% & 59.0\% & -\\
\textbf{ts(20)}& \textbf{83.0\%} & 69.8\% & 58.0\% & 82.9\%\\
\textbf{ts(50)}& \textbf{84.6\%} & 69.8\% & 58.3\% & 84.5\%\\
\textbf{fp(8)}& \textbf{90.7\%} & 81.2\% & 84.5\% & 85.5\%\\
\textbf{fp(16)}& 92.1\% & 83.3\% & 88.4\% & \textbf{93.2\%}\\
\textbf{fp(32)}& 85.4\% & 81.4\% & 88.1\% & \textbf{92.7\%}\\
\textbf{sts()}& \textbf{95.2\%} & 78.4\% & 82.5\% & -\\
\bottomrule
    \end{tabular}
    \label{tab:tab:ISCX_Encryption_table}
    \end{table}
\begin{table}[p]
    \caption{ISCX Categories classification task.}
    \centering
    \begin{tabular}{lcccc}
    \toprule
    & {\textbf{RF}} & {\textbf{SVM}} & {\textbf{LR}} & {\textbf{DEEP}} \\
    \midrule
    \textbf{dist(5)}& \textbf{89.1\%} & 88.5\% & 82.6\% & -\\
\textbf{dist(10)}& \textbf{90.6\%} & 89.5\% & 89.4\% & -\\
\textbf{dist(20)}& 91.1\% & 90.6\% & \textbf{93.3\%} & 93.2\%\\
\textbf{dist(50)}& 89.4\% & 92.0\% & 91.5\% & \textbf{94.7\%}\\
\textbf{ts(5)}& \textbf{77.3\%} & 62.4\% & 55.3\% & -\\
\textbf{ts(10)}& \textbf{77.9\%} & 68.1\% & 61.5\% & -\\
\textbf{ts(20)}& 76.7\% & 72.8\% & 64.1\% & \textbf{78.3\%}\\
\textbf{ts(50)}& 76.5\% & 75.5\% & 63.9\% & \textbf{82.7\%}\\
\textbf{fp(8)}& 85.8\% & 89.0\% & 87.6\% & \textbf{92.2\%}\\
\textbf{fp(16)}& 83.1\% & 89.7\% & 88.7\% & \textbf{93.6\%}\\
\underline{\textbf{fp(32)}}& 80.7\% & 88.2\% & 88.5\% & \textbf{94.7\%}\\
\textbf{sts()}& \textbf{92.3\%} & 82.6\% & 86.5\% & -\\
\bottomrule
    \end{tabular}
    \label{tab:tab:ISCX_Categories_table}
    \end{table}
\begin{table}[p]
    \caption{VPN Services classification task.}
    \centering
    \begin{tabular}{lcccc}
    \toprule
    & {\textbf{RF}} & {\textbf{SVM}} & {\textbf{LR}} & {\textbf{DEEP}} \\
    \midrule
    \textbf{dist(5)}& \textbf{90.3\%} & 86.5\% & 82.3\% & -\\
\textbf{dist(10)}& 97.8\% & \textbf{98.7\%} & 97.1\% & -\\
\textbf{dist(20)}& \textbf{98.9\%} & 98.6\% & 98.4\% & 98.9\%\\
\underline{\textbf{dist(50)}}& \textbf{99.7\%} & 98.6\% & 99.0\% & 99.2\%\\
\textbf{ts(5)}& \textbf{92.2\%} & 58.3\% & 36.0\% & -\\
\textbf{ts(10)}& \textbf{91.6\%} & 63.2\% & 49.0\% & -\\
\textbf{ts(20)}& \textbf{92.4\%} & 73.5\% & 60.0\% & 91.6\%\\
\textbf{ts(50)}& \textbf{91.7\%} & 74.4\% & 62.0\% & 90.2\%\\
\textbf{fp(8)}& 96.2\% & 93.2\% & 95.9\% & \textbf{97.7\%}\\
\textbf{fp(16)}& 96.7\% & 97.5\% & 97.5\% & \textbf{99.2\%}\\
\textbf{fp(32)}& 95.4\% & 97.3\% & 97.2\% & \textbf{99.5\%}\\
\textbf{sts()}& \textbf{96.2\%} & 85.7\% & 93.4\% & -\\
\bottomrule
    \end{tabular}
    \label{tab:tab:VPN_Services_table}
    \end{table}
\begin{table}[p]
    \caption{Streaming or Not classification task.}
    \centering
    \begin{tabular}{lcccc}
    \toprule
    & {\textbf{RF}} & {\textbf{SVM}} & {\textbf{LR}} & {\textbf{DEEP}} \\
    \midrule
    \textbf{dist(5)}& \textbf{82.4\%} & 75.2\% & 69.8\% & -\\
\textbf{dist(10)}& \textbf{84.1\%} & 80.0\% & 79.1\% & -\\
\textbf{dist(20)}& \textbf{82.2\%} & 79.5\% & 79.4\% & 82.1\%\\
\textbf{dist(50)}& \textbf{80.4\%} & 77.8\% & 78.5\% & 79.9\%\\
\textbf{ts(5)}& \textbf{68.1\%} & 62.1\% & 59.3\% & -\\
\textbf{ts(10)}& \textbf{69.4\%} & 65.3\% & 64.3\% & -\\
\textbf{ts(20)}& \textbf{69.9\%} & 65.1\% & 64.4\% & 63.5\%\\
\textbf{ts(50)}& \textbf{69.5\%} & 62.6\% & 63.1\% & 65.1\%\\
\textbf{fp(8)}& 79.1\% & 76.9\% & 75.9\% & \textbf{80.7\%}\\
\textbf{fp(16)}& 79.1\% & 77.1\% & 78.5\% & \textbf{82.6\%}\\
\underline{\textbf{fp(32)}}& 76.3\% & 74.5\% & 76.2\% & \textbf{84.2\%}\\
\textbf{sts()}& \textbf{80.1\%} & 64.9\% & 71.7\% & -\\
\bottomrule
    \end{tabular}
    \label{tab:tab:VPN_Strm_table}
    \end{table}
}

==> chapters/results/tables/memory_requirements.tex <==
\begin{table}[tb]
\caption{Memory requirements for representation types (for the ISCX classification tasks), with $\tau = 15s$ and a flow rate of 1 million flows per second.}
\centering
\small
\begin{tabular}{lcccc}
\toprule & {\textbf{Repr. Size (B)}}& {\textbf{Approx. Required Memory (B)}}\\ \midrule\
\textbf{dist(5)}& 20 & 300.0M\\
\textbf{dist(10)}& 40 & 600.0M\\
\textbf{dist(20)}& 80 & 1.2G\\
\textbf{dist(50)}& 200 & 3.0G\\
\textbf{ts(5)}& 30 & 450.0M\\
\textbf{ts(10)}& 60 & 900.0M\\
\textbf{ts(20)}& 120 & 1.8G\\
\textbf{ts(50)}& 300 & 4.5G\\
\textbf{fp(8)}& 128 & 1.9G\\
\textbf{fp(16)}& 512 & 7.7G\\
\textbf{fp(32)}& 2048 & 30.7G\\
\textbf{sts()}& 132 & 2.0G\\
\bottomrule
\end{tabular}
\label{tab:memory}
\end{table}

==> chapters/results/tables/throughput.tex <==
\begin{table}[tb]
    \caption{}
    \centering
    \begin{tabular}{lcccc}
    \toprule
    & {\textbf{RF}} & {\textbf{SVM}} & {\textbf{LR}} & {\textbf{DEEP}} \\
    \midrule
    \underline{\textbf{dist(2)}}& 110.8K$\frac{f}{s}$ & 8.4K$\frac{f}{s}$ & \textbf{13.7296M$\frac{f}{s}$} & -\\
\textbf{dist(5)}& 108.8K$\frac{f}{s}$ & 9.4K$\frac{f}{s}$ & \textbf{11.7904M$\frac{f}{s}$} & -\\
\textbf{dist(10)}& 99.4K$\frac{f}{s}$ & 8K$\frac{f}{s}$ & \textbf{8.7808M$\frac{f}{s}$} & -\\
\textbf{dist(50)}& 94.2K$\frac{f}{s}$ & 4.6K$\frac{f}{s}$ & \textbf{921.2K$\frac{f}{s}$} & 6.4K$\frac{f}{s}$\\
\textbf{ts(2)}& 92K$\frac{f}{s}$ & 3.8K$\frac{f}{s}$ & \textbf{9.9652M$\frac{f}{s}$} & -\\
\textbf{ts(5)}& 96.8K$\frac{f}{s}$ & 4.2K$\frac{f}{s}$ & \textbf{8.6144M$\frac{f}{s}$} & -\\
\textbf{ts(10)}& 98K$\frac{f}{s}$ & 3.8K$\frac{f}{s}$ & \textbf{7.0988M$\frac{f}{s}$} & -\\
\textbf{ts(50)}& 92.6K$\frac{f}{s}$ & 2.6K$\frac{f}{s}$ & \textbf{877.2K$\frac{f}{s}$} & 6.6K$\frac{f}{s}$\\
\textbf{sts()}& 103.4K$\frac{f}{s}$ & 5.4K$\frac{f}{s}$ & \textbf{7.4316M$\frac{f}{s}$} & -\\
\textbf{fp(8)}& 98.8K$\frac{f}{s}$ & 5.6K$\frac{f}{s}$ & \textbf{3.2988M$\frac{f}{s}$} & 6.8K$\frac{f}{s}$\\
\textbf{fp(16)}& 86.2K$\frac{f}{s}$ & 1.8K$\frac{f}{s}$ & \textbf{552.6K$\frac{f}{s}$} & 6.2K$\frac{f}{s}$\\
\textbf{fp(32)}& 62.6K$\frac{f}{s}$ & 400$\frac{f}{s}$ & \textbf{176K$\frac{f}{s}$} & 5.2K$\frac{f}{s}$\\
\bottomrule
    \end{tabular}
    \label{tab:throughput}
    \end{table}

==> chapters/results/tables/throughput_ISCX_Apps.tex <==
\begin{table}[tbh]
    \caption{Classification throughput (in flows per second, using batches of 1K representations) for the ISCX Applications classification task.}
    \centering
    \begin{tabular}{lcccc}
    \toprule
    & {\textbf{RF}} & {\textbf{SVM}} & {\textbf{LR}} & {\textbf{DEEP}} \\
    \midrule
\textbf{dist(5)}& 96.3K & 15.4K & \textbf{7.7M} & -\\
\textbf{dist(10)}& 95.7K & 13.8K & \textbf{1.7M} & -\\
\textbf{dist(20)}& 93.7K & 11.6K & \textbf{1.4M} & 9.2K\\
\textbf{dist(50)}& 89.2K & 10.1K & \textbf{894.2K} & 8.7K\\
\textbf{ts(5)}& 95.5K & 9.5K & \textbf{7.4M} & -\\
\textbf{ts(10)}& 94.2K & 9.4K & \textbf{1.8M} & -\\
\textbf{ts(20)}& 91.0K & 8.2K & \textbf{1.4M} & 9.2K\\
\textbf{ts(50)}& 84.9K & 6.1K & \textbf{937.1K} & 8.8K\\
\textbf{sts()}& 94.2K & 10.9K & \textbf{1.8M} & -\\
\textbf{fp(8)}& 91.8K & 10.1K & \textbf{1.4M} & 9.0K\\
\textbf{fp(16)}& 73.5K & 3.5K & \textbf{551.9K} & 7.8K\\
\textbf{fp(32)}& 53.3K & 766.7 & \textbf{177.6K} & 6.1K\\
\bottomrule
    \end{tabular}
    \label{tab:ISCX_Apps_throughput}
    \end{table}
